Multi-Criteria Optimal Planning for Energy Policies in CLP

In the policy making process a number of disparate and diverse issues such as economic development, environmental aspects, as well as the social acceptance of the policy, need to be considered. A single person might not have all the required expertises, and decision support systems featuring optimization components can help to assess policies. Leveraging on previous work on Strategic Environmental Assessment, we developed a fully-fledged system that is able to provide optimal plans with respect to a given objective, to perform multi-objective optimization and provide sets of Pareto optimal plans, and to visually compare them. Each plan is environmentally assessed and its footprint is evaluated. The heart of the system is an application developed in a popular Constraint Logic Programming system on the Reals sort. It has been equipped with a web service module that can be queried through standard interfaces, and an intuitive graphic user interface.

==> related.tex <==
\section{Related work}
\label{sec:related}

\marco{Marco e Michela: Related su environmental assessment, regional planning, etc.}

\elisa{Elisa: Related su Pareto}

\stefano{Stefano e Federico: Related sulla web interface}

Within the EU project \emph{No\--Miracle}, for instance, researchers from 17 different European countries have developed a methodology that exploits maps to visualise information about environmental risks with respect to the territory~\footnote{See \url{http://nomiracle.jrc.ec.europa.eu/}.}
In recent years, the Australian Government has welcomed the foundation of the Policy Visualisation Network.
The purpose of such committee is to bring policy makers and designers together, to explore how the Australian Public Service can make better use of visualisation techniques to provide better policy analysis, advice or engagement~\cite{lindquist2011surveying,lindquist2011discussion}.
